ChEX: Interactive Localization and Region Description in Chest X-rays

Report generation models offer fine-grained textual interpretations of medical images like chest X-rays, yet they often lack interactivity (i.e. the ability to steer the generation process through user queries) and localized interpretability (i.e. visually grounding their predictions), which we deem essential for future adoption in clinical practice. While there have been efforts to tackle these issues, they are either limited in their interactivity by not supporting textual queries or fail to also offer localized interpretability. Therefore, we propose a novel multitask architecture and training paradigm integrating textual prompts and bounding boxes for diverse aspects like anatomical regions and pathologies. We call this approach the Chest X-Ray Explainer (ChEX). Evaluations across a heterogeneous set of 9 chest X-ray tasks, including localized image interpretation and report generation, showcase its competitiveness with SOTA models while additional analysis demonstrates ChEX's interactive capabilities. Code: https://github.com/philip-mueller/chex

==> sections/08_conclusion.tex <==
%auto-ignore
\section{Conclusion}
We proposed ChEX, a model for predicting visually grounded textual descriptions of chest X-rays based on user queries. 
ChEX offers a unique combination of interpretability and interactivity not provided by other report generation models, while also supporting localized tasks beyond report generation.
Our analysis underscores ChEX's competitive performance against state-of-the-art models across 9 tasks, and its responsiveness to user prompts.
We hope that our work inspires further research into interactive and localized text generation models.

